INVICTUS: Optimizing Boolean Logic Circuit Synthesis via Synergistic Learning and Search

Logic synthesis is the first and most vital step in chip design. This steps converts a chip specification written in a hardware description language (such as Verilog) into an optimized implementation using Boolean logic gates. State-of-the-art logic synthesis algorithms have a large number of logic minimization heuristics, typically applied sequentially based on human experience and intuition. The choice of the order greatly impacts the quality (e.g., area and delay) of the synthesized circuit. In this paper, we propose INVICTUS, a model-based offline reinforcement learning (RL) solution that automatically generates a sequence of logic minimization heuristics ("synthesis recipe") based on a training dataset of previously seen designs. A key challenge is that new designs can range from being very similar to past designs (e.g., adders and multipliers) to being completely novel (e.g., new processor instructions). %Compared to prior work, INVICTUS is the first solution that uses a mix of RL and search methods joint with an online out-of-distribution detector to generate synthesis recipes over a wide range of benchmarks. Our results demonstrate significant improvement in area-delay product (ADP) of synthesized circuits with up to 30\% improvement over state-of-the-art techniques. Moreover, INVICTUS achieves up to $6.3\times$ runtime reduction (iso-ADP) compared to the state-of-the-art.

==> 05_Experiment_new.tex <==
\section{Evaluation}

We present our experimental setup and the efficacy of \solution{} by showing the \ac{ADP} reduction after comparing its generated recipes to %by generating better synthesis recipes compared to 
\ac{SOTA} synthesis. We use a fixed, limited run-time budget when evaluating all the methods.

\subsection{Setup}

\input{tables/table_mcnc_dataset}
\textbf{Dataset:} We consider three popular dataset primarily used in logic synthesis community for evaluating synthesis approaches: MCNC~\cite{mcnc}, EPFL arithmetic and random control benchmarks~\cite{epfl}. MCNC benchmarks contain 38 circuits ranging from 100-8k AND nodes in \ac{AIG} graphs. EPFL benchmarks are new and are of two different types: arithmetic and random control. Arithmetic circuits are datapath intensive designs performing arithmetic operations. We consider 9 EPFL arithmetic benchmarks with nodes in \ac{AIG} ranging from 1k-44k. On the other hand, random control circuits are mostly control logic circuits consisting of controller, finite-state machines, routers and random function etc. For our experiments, we consider 9 random control circuits with nodes varying in the range of 100-46k nodes.

\textbf{RL agents and train-test split:} Our train-test split criteria is motivated from prior work~\cite{fu2020d4rl}. We train dataset-specific \ac{RL} agents to evaluate performance of \solution{}. The key reason is: circuits vary structurally and functionally a lot accross various dataset. Training domain-specific agents for each dataset ensure that the test designs have certain characterization similar to the training data:
\begin{enumerate}  [noitemsep,nolistsep,leftmargin=0.5cm]
    \item \textbf{MCNC agent:} We divide MCNC dataset circuits into three set: training, validation and test set. The training set contains 14 circuits; validation and test data consists of 12 circuits each. We perform train-test split with the intuition: circuits performing similar operation but with certain variation (e.g. increasing complexity) have been divided in train and test set. We train one agent as there are sufficient number of circuits for training, validation and test.
    \item \textbf{EPFL arithmetic:} We divide nine arithmetic circuits into three sets of 7-2 split (arithmetic agents I, II and III) and one set of 6-3 split (arithmetic agent IV) and train \ac{RL} agents. The primary reason for training multiple agents is dataset scarcity. The splits are done randomly. For validation data, we augment training data with training circuits combined with unseen circuits (\texttt{alu2} and \texttt{apex7}). We also used four random control circuits as validation data. We use validation data to set the threshold of cosine distance which is our \ac{OOD} hyperparameter. We test our arithmetic agents on tes circuits and remaining random control circuits.
    \item \textbf{EPFL random control:} Similar to arithmetic benchmarks, we divide random control benchmarks into four 7-2 split and one 8-1 split and train five \ac{RL} agents. We create validation data following the above strategy. We also use four arithmetic benchmarks for validation and five for testing.
\end{enumerate}

\textbf{Objective metric/return:} We synthesize the \ac{AIG} with a synthesis recipe, perform technology mapping using ASAP 7nm technology library and collect area and delay values. Consistent with prior works, we use area-delay product as evaluation metric and use \texttt{resyn2}'s area-delay product as baseline. We report area-delay product reduction (\%) over \texttt{resyn2}'s baseline \ac{ADP} and compare it with prior \ac{SOTA} methods~\cite{neto2022flowtune,bullseye}.


\textbf{Training details and hyper-parameters:} We present our network architecture in ~\autoref{fig:networkArchitecture}. We use \textit{He initialization} to initialize the weights of our agent network. Following~\cite{googleRLempirical}, we multiply the weights of the final layer with $0.01$ to prevent bias towards any action. We train our agents for $50$ epochs. We used the Adam optimizer set the initial learning rate to $0.01$.

In each epoch, we perform MCTS on each circuit. The MCTS search budget($K$) is set to $512$ at each level of synthesis. We keep the synthesis recipe length $L=10$, thus we perform MCTS up to search tree depth $10$. At each level, the replay buffer stores the best experience tuple having information about the state and action probability distribution scores collected from monte carlo rollout.

% the MCTS search budget $K$ is set to 2048. For each design in the training set, we perform an MCTS search and update the replay buffer with experience tuples that include information about the state, the monte carlo rollout values for each action, and the action probability distribution of the MCTS policy. As the recipe length is $L=10$, we store the best experience tuple in the replay buffer at every depth of exploration up to 10.

After performing MCTS simulations on training circuits, we sample $|$\textit{Training circuits}$|*L$ experiences from the replay buffer and train the agent. The \ac{RL} agent minimizes the cross entropy loss between $\pi_\theta$ and the MCTS agent $\pi_{MCTS}$. We set the replay buffer size to $|$\textit{Training circuits}$|*L*2$. The agent training time for MCNC benchmarks took around 27 hours however EPFL arithemetic and random control agents took ~7 days. We performed the training on a server machine having Ubuntu 20.04 and one NVIDIA RTX A4000 having 16GB VRAM. We used Yosys, ABC and Pytorch-geometric for end-to-end implementation.

\textbf{Evaluation:} We compare \solution{} with three main methods: standard \ac{MCTS}~\cite{neto2022flowtune}; simulated annealing(SA) with \ac{QoR} predictor~\cite{bullseye} and on-policy \ac{RL}-based approach~\cite{mlcad_abc}. Standard MCTS~\cite{neto2022flowtune} and SA with QoR Predictor~\cite{bullseye} are the current \ac{SOTA} work for area-delay optimization. \cite{neto2022flowtune} employs Monte-carlo tree search guided logic synthesis wheras \cite{bullseye} build a zero-shot predictor model and fine-tunes it on circuit under consideration and use simulated annealing to generate synthesis recipes. \cite{mlcad_abc} use an on-policy \ac{RL} using Graph neural network for recipe generation.

\input{tables/table_mcnc}
During evaluation, we set synthesis run budget as $100$ for all techniques. We use \ac{ADP} of \texttt{resyn2} as baseline to measure effectiveness of a synthesis recipe for ADP reduction. \solution{} uses design embedding based \ac{OOD} detector to determine the percentage of pre-trained agent recommendation to be used for tuning the search.
Design embedding based \ac{OOD} detector first computes the minimum cosine distance of each validation circuit from training circuits and perform a labeling of 0 or 1; 0 being agent+MCTS wins whereas 1 means standard MCTS wins. It then sets the threshold value $\delta_{th}$ based on area under ROC. Post that, for a new unseen circuit (test data), we set $\alpha$ using ~\autoref{eq:alpha-factor}. For MCNC circuits, we obtained $\delta_{th}=0.007$ and temperature $T=0.006$. $\alpha$ sets the amount of biasness of \ac{MCTS} using pre-trained \ac{RL} agent. 

%We call this zero effort OOD detector: We upfront choose \solution{}'s choice to pick either monte-carlo tree search or agent guided search.

%\solution{} uses design embedding based \ac{OOD} detector for determining whether to deploy RL+MCTS agent during search or not. Design embedding based \ac{OOD} detector first computes the minimum cosine distance of each validation circuit from training circuits and perform a labeling of 0 or 1; 0 being RL+MCTS wins wheras 1 means standard MCTS wins. It then sets the threshold value $T$ based on area under ROC. Post that, for a new unseen circuit (test data), we set $\alpha$ to 0 or 1 by comparing minimum cosine distance with the threshold value $T$. Depending on the value of $\alpha$, our algorithm chooses whether to use \ac{RL} agent or not. We call this zero effort OOD detector: We upfront choose \solution{}'s choice to pick either monte-carlo tree search or agent guided search.


%based on cosine similarity embedding and comparing it with threshold temperature value. 

%The second approach is: Synthesis effort based approach. This is similar to the user based knob provided by commercial synthesis tools as \textit{low}, \textit{medium} and \textit{high} effort synthesis.  We set a hyper-parameter $K$: number of iterations for which both search techniques continue to explore better synthesis recipes. After $K$ iterations, we choose the winner and continue the search till $N^{th}$ iteration, stopping the other thread. We set $K$=$20$, $40$ and $60$ corresponding to low, medium and high effort. Thus, high effort indicates synthesis run-budget of $160$ and picking the most   likely winner thread at the expense of additional synthesis runs.



\subsection{Results}

% \begin{figure}[t]
% \centering
%    \subfloat[alu4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_alu4_compare_ADP_best_alu4.pdf} }}%
% 	}
% 	\subfloat[apex1]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_apex1_compare_ADP_best_apex1.pdf} }}
% 	}
%         \subfloat[apex2]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_apex2_compare_ADP_best_apex2.pdf} }}
% 	}
% 	\subfloat[apex4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_apex4_compare_ADP_best_apex4.pdf} }}
% 	}
% \vspace{-0.2in}
% 	\subfloat[b9]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_b9_compare_ADP_best_b9.pdf} }}}
%         \subfloat[c880]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_c880_compare_ADP_best_c880.pdf} }}
% 	}
% 	\subfloat[prom1]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_prom1_compare_ADP_best_prom1.pdf} }}
% 	}
% 	\subfloat[i9]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_i9_compare_ADP_best_i9.pdf} }}}
% \vspace{-0.2in}
%         \subfloat[m4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_m4_compare_ADP_best_m4.pdf} }}
% 	}
%          \subfloat[pair]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_pair_compare_ADP_best_pair.pdf} }}
% 	}
%         \subfloat[max1024]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_max1024_compare_ADP_best_max1024.pdf} }}
% 	}
%         \subfloat[c7552]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mcnc_c7552_compare_ADP_best_c7552.pdf} }}
% 	}
% 	%\vspace{0.3in}
%     \caption{Area-delay product reduction (in \%) compared to resyn2 on MCNC circuits. \solution{} classified \texttt{c7552}, \texttt{pair} and \texttt{max1024} as out-of-distribution samples for MCNC agent and picked standard search (Flowtune). For rest of the circuits, \solution{} used Agent+MCTS(GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING)}
%     \label{fig:performance-mcnc}
% \end{figure}


\begin{figure}[t]
\centering
   \subfloat[alu4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_alu4_compare_ADP_best_alu4.pdf} }}%
	}
	\subfloat[apex1]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_apex1_compare_ADP_best_apex1.pdf} }}
	}
        \subfloat[apex2]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_apex2_compare_ADP_best_apex2.pdf} }}
	}
	\subfloat[apex4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_apex4_compare_ADP_best_apex4.pdf} }}
	}
\vspace{-0.2in}
	\subfloat[b9]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_b9_compare_ADP_best_b9.pdf} }}}
        \subfloat[c880]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_c880_compare_ADP_best_c880.pdf} }}
	}
	\subfloat[prom1]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_prom1_compare_ADP_best_prom1.pdf} }}
	}
	\subfloat[i9]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_i9_compare_ADP_best_i9.pdf} }}}
\vspace{-0.2in}
        \subfloat[m4]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_m4_compare_ADP_best_m4.pdf} }}
	}
         \subfloat[\color{red}{pair$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_pair_compare_ADP_best_pair.pdf} }}
	}
        \subfloat[\color{red}{max1024$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_max1024_compare_ADP_best_max1024.pdf} }}
	}
        \subfloat[\color{red}{c7552$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mcnc_c7552_compare_ADP_best_c7552.pdf} }}
	}
	%\vspace{0.3in}
    \caption{Area-delay product reduction (in \%) compared to resyn2 on MCNC circuits. \solution{} classified \texttt{c7552}, \texttt{pair} and \texttt{max1024} as out-of-distribution samples for MCNC agent and picked standard search (Flowtune). For rest of the circuits, \solution{} used Agent+MCTS(GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING)}
    \label{fig:performance-mcnc}
\end{figure}



We now discuss the performance of \solution{} in reducing area-delay product over existing state-of-the-art approaches. We categorically describe the performance of our agents on our dataset circuits.

% \textbf{Performance on MCNC benchmarks:} ~\autoref{fig:performance-mcnc} shows the effectiveness of agent+MCTS generated recipes over Flowtune(\ac{SOTA}) in \ac{ADP} reduction over 100 iterations. On 9 out of 12 benchmarks, MCTS guided by pre-trained agents help generate better recipes than Flowtune (standard MCTS), with substantially outperforming on benchmarks like \texttt{alu4, apex2, i9, m4, prom1} and \texttt{c880}. In \texttt{alu4}, after 20th iteration, search with pre-trained agent explored better rewarding paths whereas flow-tune continued searching for better paths thus showing no further improvement. We observe similar trend for \texttt{apex2, m4, prom1} and \texttt{c880} where flow-tune after showing some initial progress got stuck in exploring better paths. This shows: pre-trained agent helps bias search towards better rewarding paths essentially leading to better \ac{ADP} reduction in fixed synthesis runtime constraints. For remaining three benchmarks \texttt{c7552, pair} and \texttt{max1024}, flowtune achieved better \ac{ADP} than agent+MCTS guided search. 

% In ~\autoref{tab:qorMCNC}, we reported overall ADP reduction of obtained by \solution{} generated recipes. \solution{} intelligently chooses whether to use pre-trained agent for MCTS or perform standard
% MCTS using out-of-distribution detection. Using cosine distance based \ac{OOD}, we obtained the threshold temperature $T=0.005$ using validation data circuits. Using $T=0.005$, \solution{} classify \texttt{pair} and \texttt{max1024} as \ac{OOD} samples and do not use pre-trained agent during MCTS search. \solution{} using cosine distance based OOD obtains best ADP reduction in 11 out 12 benchamrks by correctly classifying all the nine samples as in-distribution (deploys Agent+MCTS) and two out of three as out-of-distribution samples (deploys standard MCTS). \solution{} using low effort synthesis ($K=20$) are able to pick the winning search mechanism in 11 out of 12 benchmarks. The exception is with \texttt{m4} benchmark where post 20th iteration, standard MCTS return were better than agent+MCTS return which later saturated. In mid and high effort based \ac{OOD} detection, \solution{} picked the winning search with 100\% success indicating that \solution{} is correctly able to leverage to agent+MCTS search when unseen design bears similarity with training data and/or the intuition that agent+MCTS based search result in better returns quickly for unseen designs bearing similarity with past designs.

\textbf{Performance on MCNC benchmarks:} \autoref{fig:performance-mcnc} shows ADP reduction of \solution{} generated recipes over MCTS-based SOTA method~\cite{neto2022flowtune}. We observe that agent guided search($\alpha=1$) on 9 out of 12 benchmarks. On, \ac{OOD} benchmarks namely \texttt{pair, max1024} and \texttt{c7552}, SOTA method~\cite{neto2022flowtune}(standard search) outperforms agent guided search. Compared to that, our soft OOD based search outperforms \cite{neto2022flowtune} on all the benchmarks with substantially out-performing on ($\sim5-7\%$) on benchmarks such as \texttt{i9, prom1}, and \texttt{c880} on in-distribution design and up to $3.7\%$ improvement on out-of-distribution design(\texttt{pair}). Our soft OOD based approach beating standard MCTS method provides us an insight: biasing search upto a certain degree using pre-trained agent on \ac{OOD} samples still helps pruning away bad paths. On the contrary, we also observe on most of our in-distribution designs; our soft OOD based approach achieved the same ADP reduction (except \texttt{alu4} and \texttt{m4}). These two designs have the least cosine distances indicates that these two designs gets heavily benefited from agent-guided search. On the contrary, in distribution samples like \texttt{apex1}, \texttt{apex4} are closer to $\delta_{th}$ values; thus \ac{ADP} reduction improved over both techniques: 1) agent-based search, and 2) MCTS search.

In Table~\ref{tab:qorMCNC}, we compare \ac{ADP} reduction obtained by the \solution{} with prior \ac{SOTA} methods. \cite{mlcad_abc} uses online \ac{RL} to generate synthesis recipes; \cite{bullseye} learns a synthesis recipe predictor model and use it as an evaluator via simulated annealing (SA+Pred.). \textbf{\solution{} wins on $11$ out of $12$ benchmarks with an overall geomean \ac{ADP} reduction of 20.41\%. This is $+7.61\%$, $+3.07\%$ and $+3.75\%$ improvement over online RL~\cite{mlcad_abc}, SA+Predictor model~\cite{bullseye}  and standard MCTS search ~\cite{neto2022flowtune} approaches.}

% and as high as $\sim+7\%$ reduction(\texttt{i9}).

% solution{} tunes the $\alpha$ whether to use a pre-trained agent for MCTS or perform standard MCTS using out-of-distribution detection. Using cosine distance-based \ac{OOD} detection, a threshold temperature $T=0.005$ was obtained using validation data circuits. Using this value of $T$, \solution{} classifies \texttt{pair} and \texttt{max1024} as \ac{OOD} samples and does not use a pre-trained agent during MCTS search. With cosine distance-based OOD detection, \solution{} obtains the best \ac{ADP} reduction in 11 out of 12 benchmarks by correctly classifying all nine samples as in-distribution (deploys Agent+MCTS) and two out of three as out-of-distribution samples (deploys standard MCTS). \textbf{Overall, \solution{} achieved geomean \ac{ADP} reduction of 19\% with cosine-based \ac{OOD} detection. }

\input{tables/table_epfl_arith}

\textbf{Performance on EPFL arithmetic benchmarks:} 

We evaluate \ac{ADP} reduction on EPFL arithmetic benchmarks with each evaluated by agent trained on other benchmarks. In ~\autoref{fig:performance-epfl-arith}, we observe that \ac{ADP} reduction of agent-based search is better than standard search~\cite{neto2022flowtune} on all benchmarks except \texttt{square}. This indicates that circuits used in pre-training the agents have similar characterization as test data circuits. Recipes generated using agent-guided search ($\alpha=1$) achieve substantial ADP reduction (upto $\sim$11\%) on benchmarks like \texttt{bar, div} and \texttt{max} over standard MCTS ($\alpha=0$) . For benchamrks like \texttt{bar, div, log2} and \texttt{multiplier}, agent-guided search outperform \ac{ADP} of standard MCTS generated recipe. For \texttt{adder} where agent guided search achieved same \ac{ADP} reduction as that of standard MCTS, we get $2.2\times$ run-time improvement. However, for \texttt{square}, standard MCTS performs better than agent guided search.

%Agent+MCTS search outperform Bulls-eye on all arithemetic benchmarks. For \texttt{adder} and \texttt{bar}, Agent+MCTS search achieved same \ac{ADP} reduction in 50.2\% and 9.4\% lesser time compared to Bulls-eye.  

We present \ac{ADP} reduction by \solution{} generated recipes on arithmetic circuits in ~\autoref{tab:qorEPFLarith}. For each of the arithmetic agents, we used  cosine based \ac{OOD} detection to determine temperature threshold $T$ using validation data circuits. Except \texttt{square}, each benchmark were classified as in-distribution and agent+MCTS search is picked to generate synthesis recipe. Our cosine-based OOD correctly classified all the benchmarks resulting in best \ac{ADP} reduction recipe. 

\textbf{Overall, \solution{} achieved geomean \ac{ADP} reduction of $22.07\%$ with cosine-based \ac{OOD} detection. This results in $+5.52\%$ and $+6.93\%$ improvement over Flowtune~\cite{neto2022flowtune} and Bullseye~\cite{bullseye} and as high as $\sim+10\%$ and $\sim+30\%$ reduction(\texttt{div}) over Flowtune and Bullseye.}

\input{tables/table_epfl_rc}
\textbf{Performance on EPFL random control benchmarks:} \autoref{fig:performance-epfl-rc} compares the performance of \ac{RL} agent guided MCTS versus Flowtune for \ac{ADP} reduction. Contrary to MCNC and EPFL arithmetic benchmarks, we surprisingly observe that random-control agents could only achieve better \ac{ADP} reduction on four out of nine benchmarks. This correlates with EPFL random control benchmark characterization~\cite{epfl} having a wide variation in circuit structure and functionality~. Thus, synthesis recipes behave differently on each circuit leading to train test distribution shift. Hence, pre-trained random control agents tend to bias the search towards bad paths which appears to be rewarding by the agents. On the other hand, Flowtune (standard MCTS) and Bullseye fared better on rest of the benchmarks.

\solution{} alleviates this problem of using \ac{RL}-guided MCTS using cosine-based \ac{OOD} detection. In ~\autoref{fig:performance-epfl-rc}, we observe that \solution{} successfully classify seven out of nine benchmarks about deploying \ac{RL} agent using MCTS. Thus, \solution{} generates best \ac{ADP} reduction recipes for seven out of nine benchmarks. Relying solely on agent based search only achieve best results on five out of nine designs. This highlights the contribution of using \ac{OOD}-based classification where synthesis runs are expensive and knowing upfront is important whether \ac{RL}-guided agent is really going be beneficial compared to standard search (Flowtune). \textbf{Overall, \solution{} achieved geomean \ac{ADP} reduction of 10.80\% with cosine-based \ac{OOD} detection. This accounts for $+0.42\%$ and $+0.33\%$ improvement over Flowtune~\cite{neto2022flowtune} and Bullseye~\cite{bullseye} and as high as $\sim+3.27\%$ and $\sim+5.0\%$ reduction(\texttt{div}) over Flowtune and Bullseye.}

% we observe \solution{} used pre-trained agents for all the benchmarks except \texttt{}

% We evaluated the quality of the synthesis recipe generated by standard MCTS and MCTS with a pre-trained agent by comparing the improvement in area-delay product (ADP) to that of \texttt{resyn2}. For example, in \autoref{fig:performance-set1}a, the MCTS+prior generated synthesis recipe for \texttt{adder} with 1.23x improvement in ADP over \texttt{resyn2} in 18 iterations. The legend in the figure indicates whether the \solution{} used the pre-trained agent during the search. As shown in \autoref{fig:performance-set1}, we can see that \solution{} used pre-trained agent in MCTS resulted in better ADP improvement for 7 out of 8 designs compared to vanilla MCTS. On \texttt{adder}, both methods resulted in the same improvement. However, MCTS+Prior generated the recipe in 18 iterations, while vanilla MCTS took around 50 iterations on average, resulting in a 2.7x improvement in runtime. In terms of ADP, the recipe generated by MCTS+Prior yielded  a 2-40\% improvement over the recipe generated by standard MCTS for designs that the agent was trained on. 

% We observe in ~\autoref{fig:performance-set2} that using a pre-trained agent in MCTS improved results compared to vanilla MCTS. This suggests that the sequence of transformations learned during training can also benefit new, unseen circuits. These findings demonstrate that a pre-trained agent can aid in selecting better paths during MCTS exploration, even when only a portion of the circuit was seen during training. Except \texttt{multiplier+apex7}, \solution{} generated recipe resulted in 3\%-80\% average ADP improvement compared to vanilla MCTS generated recipe. For \texttt{multiplier+apex7}, vanilla MCTS and MCTS+prior generated synthesis recipe of same ADP performance withing $K=90$ simulation budget. However, MCTS+prior was 4.5x faster in generating same quality recipe.

%In ~\autoref{fig:performance-set3}, we observe the performance of \solution{} on completely unseen hardware designs. Based on the cosine similarity, $\alpha$ is set and \solution{} chose MCTS+prior for three designs: \texttt{ctrl, i2c} and \texttt{mem\_ctrl} and vanilla MCTS for the rest. For \texttt{ctrl} and \texttt{i2c}, \solution{} generated better recipe compared to vanilla MCTS, whereas for \texttt{mem\_ctrl}, \solution{} chose MCTS+prior whose synthesis recipe is 1.5\% worse than standard MCTS. For designs where \solution{} chose MCTS over MCTS+prior, only on \texttt{int2float} MCTS+prior performed better yet cosine similarity post scaling set $\alpha=0$. However, the ADP improvement of recipe generated by MCTS+prior over MCTS is around 0.8\%. On rest of the designs like \texttt{cavlc, priority, router} and \texttt{voter}, \solution{} generated recipe following vanilla MCTS resulted in 0.7\%-90\% ADP improvement over MCTS+prior generated recipe. These show that \solution{} has successfully been able to identify when to include pre-trained agent for MCTS to explore better paths.

% The performance of the \solution{} on previously unseen hardware designs is shown in Figure~\ref{fig:performance-set3}. Based on cosine similarity, the value of $\alpha$ was determined and \solution{} chose to use MCTS+prior for three designs (\texttt{ctrl, i2c} and \texttt{mem\_ctrl}) and vanilla MCTS for the rest. For \texttt{ctrl} and \texttt{i2c}, \solution{} generated a better recipe than vanilla MCTS, however, for \texttt{mem\_ctrl} the recipe generated by \solution{} was 1.5\% worse than that of vanilla MCTS. In cases where \solution{} chose to use MCTS over MCTS+prior, only on \texttt{int2float} MCTS+prior performed better. However, the ADP improvement of the recipe generated by MCTS+prior over MCTS is around 0.8\%. On the remaining designs like \texttt{cavlc, priority, router} and \texttt{voter}, the recipe generated by \solution{} following vanilla MCTS resulted in 0.7\%-90\% ADP improvement over the recipe generated by MCTS+prior. These results show that \solution{} has successfully been able to identify when to include the pre-trained agent for MCTS in order to explore better paths.


% \begin{figure}[t]
% \centering
%    \subfloat[adder]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_adder_compare_ADP_best_adder.pdf} }}%
% 	}
% 	\subfloat[bar]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_bar_compare_ADP_best_bar.pdf} }}
% 	}
%         \subfloat[div]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_div_compare_ADP_best_div.pdf} }}
% 	}
% 	\subfloat[log2]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_log2_compare_ADP_best_log2.pdf} }}
% 	}
	
% %\vspace{-0.2in}
% 	\subfloat[max]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_max_compare_ADP_best_max.pdf} }}
% 	}
% 	\subfloat[multiplier]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_multiplier_compare_ADP_best_multiplier.pdf} }}
% 	}
%         \subfloat[sqrt]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_sqrt_compare_ADP_best_sqrt.pdf} }}
% 	}
% 	\subfloat[square]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_square_compare_ADP_best_square.pdf} }}
% 	}
% 	%\vspace{0.3in}
%     \caption{Area-delay product reduction (in \%) compared to resyn2 on EPFL arithmetic benchmarks. We evaluated \texttt{bar} and \texttt{square} with arithmetic agent I, \texttt{adder}, \texttt{sqrt} and \texttt{log2} with arithmetic agent II, \texttt{multiplier} and \texttt{sin} with arithmetic agent III and \texttt{div} and \texttt{max} with arithmetic agent IV. GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING}
%     \label{fig:performance-epfl-arith}
% \end{figure}

\begin{figure}[t]
\centering
   \subfloat[adder]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_adder_compare_ADP_best_adder.pdf} }}%
	}
	\subfloat[bar]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_bar_compare_ADP_best_bar.pdf} }}
	}
        \subfloat[div]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_div_compare_ADP_best_div.pdf} }}
	}
	\subfloat[log2]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_log2_compare_ADP_best_log2.pdf} }}
	}
	
%\vspace{-0.2in}
	\subfloat[max]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_max_compare_ADP_best_max.pdf} }}
	}
	\subfloat[multiplier]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_multiplier_compare_ADP_best_multiplier.pdf} }}
	}
        \subfloat[sqrt]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_sqrt_compare_ADP_best_sqrt.pdf} }}
	}
	\subfloat[\color{red}{square$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_square_compare_ADP_best_square.pdf} }}
	}
	%\vspace{0.3in}
    \caption{Area-delay product reduction (in \%) compared to resyn2 on EPFL arithmetic benchmarks. We evaluated \texttt{bar} and \texttt{square} with arithmetic agent I, \texttt{adder}, \texttt{sqrt} and \texttt{log2} with arithmetic agent II, \texttt{multiplier} and \texttt{sin} with arithmetic agent III and \texttt{div} and \texttt{max} with arithmetic agent IV. GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING}
    \label{fig:performance-epfl-arith}
\end{figure}



% \begin{figure}[t]
% \centering
%    \subfloat[cavlc]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_cavlc_compare_ADP_best_cavlc.pdf} }}%
% 	}
% 	\subfloat[ctrl]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_ctrl_compare_ADP_best_ctrl.pdf} }}
% 	}
%         \subfloat[int2float]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_int2float_compare_ADP_best_int2float.pdf} }}
% 	}
% 	\subfloat[i2c]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_i2c_compare_ADP_best_i2c.pdf} }}
% 	}
	
% \vspace{0.2in}
% 	\subfloat[mem\_ctrl]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_mem_ctrl_compare_ADP_best_mem_ctrl.pdf} }}%
% 	}
% 	\subfloat[priority]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_priority_compare_ADP_best_priority.pdf} }}
% 	}
%         \subfloat[router]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_router_compare_ADP_best_router.pdf} }}
% 	}
% 	\subfloat[voter]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/2023_neurips_plot_voter_compare_ADP_best_voter.pdf} }}
% 	}
% 	%\vspace{0.3in}
%     \caption{Area-delay product reduction (in \%) compared to resyn2 on EPFL random control benchmarks. Except \texttt{router}, our OOD detector successfully identified the average winner approach.GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING}
%     \label{fig:performance-epfl-rc}
% \end{figure}

\begin{figure}[t]
\centering
   \subfloat[\color{red}{cavlc$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_cavlc_compare_ADP_best_cavlc.pdf} }}%
	}
	\subfloat[ctrl]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_ctrl_compare_ADP_best_ctrl.pdf} }}
	}
        \subfloat[\color{red}{int2float$^*$}]{{{\includegraphics[width=0.27\columnwidth, valign=c]{figures/synergy_plot_int2float_compare_ADP_best_int2float.pdf} }}
	}
	\subfloat[i2c]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_i2c_compare_ADP_best_i2c.pdf} }}
	}
	
\vspace{0.2in}
	\subfloat[mem\_ctrl]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_mem_ctrl_compare_ADP_best_mem_ctrl.pdf} }}%
	}
	\subfloat[priority]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_priority_compare_ADP_best_priority.pdf} }}
	}
        \subfloat[\textcolor{red}{router$^*$}]{{{\includegraphics[width=0.27\columnwidth, valign=c]{figures/synergy_plot_router_compare_ADP_best_router.pdf} }}
	}
	\subfloat[\color{red}{voter$^*$}]{{{\includegraphics[width=0.25\columnwidth, valign=c]{figures/synergy_plot_voter_compare_ADP_best_voter.pdf} }}
	}
	%\vspace{0.3in}
    \caption{Area-delay product reduction (in \%) compared to resyn2 on EPFL random control benchmarks. Except \texttt{router}, our OOD detector successfully identified the average winner approach.GREEN: PURE LEARNING, BLUE: PURE SEARCH, ORANGE: BULLS-EYE, RED: SEARCH+LEARNING}
    \label{fig:performance-epfl-rc}
\end{figure}

\subsection{Ablation studies}
\input{tables/table_ablation}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

